Control-flow anomaly detection by process mining-based feature extraction and dimensionality reduction

The business processes of organizations may deviate from normal control flow due to disruptive anomalies, including unknown, skipped, and wrongly-ordered activities. To identify these control-flow anomalies, process mining can check control-flow correctness against a reference process model through conformance checking, an explainable set of algorithms that allows linking any deviations with model elements. However, the effectiveness of conformance checking-based techniques is negatively affected by noisy event data and low-quality process models. To address these shortcomings and support the development of competitive and explainable conformance checking-based techniques for control-flow anomaly detection, we propose a novel process mining-based feature extraction approach with alignment-based conformance checking. This variant aligns the deviating control flow with a reference process model; the resulting alignment can be inspected to extract additional statistics such as the number of times a given activity caused mismatches. We integrate this approach into a flexible and explainable framework for developing techniques for control-flow anomaly detection. The framework combines process mining-based feature extraction and dimensionality reduction to handle high-dimensional feature sets, achieve detection effectiveness, and support explainability. The results show that the framework techniques implementing our approach outperform the baseline conformance checking-based techniques while maintaining the explainable nature of conformance checking. We also provide an explanation of why existing conformance checking-based techniques may be ineffective.

==> old_sections/background.tex <==
\section{Preliminaries}
\label{sec:background}

Following is a review of techniques for implementing control-flow anomaly detection's Phase 1) and 2), focusing on ML/DL, PM, and the combination of PM and ML. Moreover, key concepts for control-flow anomaly detection are formally defined, such as event logs, sublogs, fitness, and alignments. Finally, we describe our feature extraction proposal based on alignment-based CC.

\subsection{Machine Learning and Deep Learning}
Arguably, ML provides the most commonly applied techniques for control-flow anomaly detection, implementing several learning paradigms, which can be characterized as supervised, semi-supervised, or unsupervised \cite{witten2017dmml}. Among these, the unsupervised paradigm has gained large interest due to the scarcity of labeled datasets and zero-day anomalies, employing several approaches, such as distance-based methods, e.g., kNN and clustering, and dimensionality reduction-based methods, e.g., the Principal Component Analysis (PCA) and the Autoencoder (AE) \cite{zoppi2021unsupervisedad,sakurada2014adeutoencoders}.

Recently, DL by means of RNNs and their variants, such as LSTMs and GRUs, has been used for control-flow anomaly detection, leading to satisfactory performance \cite{nolle2022binet, lahann2022lstmadpi}. However, the complexity, costly training, and explainability of DL techniques' detection results represent major challenges \cite{wang2022dlspatiotemporaldm,chen2022efficientrnntraining}. 

It is worth noting that due to ML being rooted in statistics \cite{witten2017dmml}, these approaches require the encoding of event logs into numerical data by feature extraction, such as counting the frequencies of activities in event logs, using specific embeddings such as word2vec, or computing N-grams \cite{ko2023adsystematicreview}.



==> sections/acknowledgement.tex <==
% use section* for acknowledgment
\ifCLASSOPTIONcompsoc
  % The Computer Society usually uses the plural form
  \section*{Acknowledgments}
\else
  % regular IEEE prefers the singular form
  \section*{Acknowledgment}
\fi


The authors would like to thank...

==> sections/biographies.tex <==
\begin{IEEEbiography}[{\includegraphics[height=1.25in]{images/authors/VITALE.jpg}}]{Francesco Vitale} is a PhD student in Information Technology and Electrical Engineering at the Department of Electrical Engineering and Information Technology of the University of Naples Federico II, where he has earned his M.Sc. degree in Computer Engineering in 2021. He has been a Visiting researcher at the Chair of Process and Data Science (PADS) - RWTH Aachen University in 2023. His research activities mainly address Industry 4.0, Anomaly Detection, and Process Mining.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[height=1.25in]{images/authors/PEGORARO.png}}]{Marco Pegoraro} is a Scientific Assistant (PhD
candidate) at the Chair of Process and Data Science (PADS) - RWTH Aachen University. He joined the chair in 2018. In 2016, he completed his M.Sc. degree in Computer Science at the University of Padua, Italy. His specialization is process mining, and he is particularly active in the fields of process mining in healthcare and analysis of uncertain, probabilistic, and non-deterministic data.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[height=1.25in]{images/authors/AALST.png}}]{Wil M. P. van der Aalst} is a Full professor at RWTH Aachen University, leading the Process and Data Science (PADS) group. He is also the Chief Scientist at Celonis, part-time affiliated with the Fraunhofer FIT, and a member of the Board of Governors of Tilburg University. He also has unpaid professorship positions at Queensland University of Technology (since 2003) and the Technische Universiteit Eindhoven (TU/e). Currently, he is also a distinguished fellow of Fondazione Bruno Kessler (FBK) in Trento, deputy CEO of the Internet of Production (IoP) Cluster of Excellence, and co-director of the RWTH Center for Artificial Intelligence.

\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[height=1.25in]{images/authors/MAZZOCCA.png}}]{Nicola Mazzocca} is a Full Professor of Computer Systems at the Department of Electrical Engineering and Information Technology of the University of Naples Federico II. Since 1994, he has held numerous university courses and has been involved in several professional training activities on different topics, including high-performance systems, distributed and embedded systems, security, and reliability. His research activities concern computer architecture, distributed systems, high-performance computing, and safety-critical applications. He is author of more than 250 publications in international journals, books, and conference proceedings.
\end{IEEEbiography}
\vfill
